Bundle Choice Model with Endogenous Regressors: An Application to Soda Tax

This paper proposes a Bayesian factor-augmented bundle choice model to estimate joint consumption as well as the substitutability and complementarity of multiple goods in the presence of endogenous regressors. The model extends the two primary treatments of endogeneity in existing bundle choice models: (1) endogenous market-level prices and (2) time-invariant unobserved individual heterogeneity. A Bayesian sparse factor approach is employed to capture high-dimensional error correlations that induce taste correlation and endogeneity. Time-varying factor loadings allow for more general individual-level and time-varying heterogeneity and endogeneity, while the sparsity induced by the shrinkage prior on loadings balances flexibility with parsimony. Applied to a soda tax in the context of complementarities, the new approach captures broader effects of the tax that were previously overlooked. Results suggest that a soda tax could yield additional health benefits by marginally decreasing the consumption of salty snacks along with sugary drinks, extending the health benefits beyond the reduction in sugar consumption alone.

==> tables/elasticities_TI_FA_Endo.tex <==
\begin{tabular}{llcccccc}
\hline
\multicolumn{2}{r}{Good $k=$} & 1     & 2     & 3     & 4     & 5     & 6 \bigstrut[t]\\
\multicolumn{1}{l}{Price $j=$} &       & AB InBev & Boston Beer & Heineken & MillerCoors & Other Vendors & Malt Beverage \bigstrut[b]\\
\hline
\multicolumn{1}{l}{1} & \multicolumn{1}{l}{AB InBev} & -1.058*** & -0.060 & -0.018 & -0.033 & -0.030 & -0.041 \bigstrut[t]\\
      &       & (0.320) & (0.078) & (0.102) & (0.025) & (0.023) & (0.049) \\
\multicolumn{1}{l}{2} & \multicolumn{1}{l}{Boston Beer} & -0.024 & -2.230*** & -0.028 & 0.002 & -0.011 & 0.004 \\
      &       & (0.026) & (0.691) & (0.098) & (0.016) & (0.018) & (0.034) \\
\multicolumn{1}{l}{3} & \multicolumn{1}{l}{Heineken} & -0.005 & -0.017 & -2.216*** & -0.005 & 0.001 & -0.010 \\
      &       & (0.021) & (0.060) & (0.715) & (0.013) & (0.013) & (0.030) \\
\multicolumn{1}{l}{4} & \multicolumn{1}{l}{MillerCoors} & -0.046 & 0.006 & -0.026 & -0.789*** & -0.019 & -0.054 \\
      &       & (0.036) & (0.072) & (0.090) & (0.238) & (0.023) & (0.051) \\
\multicolumn{1}{l}{5} & \multicolumn{1}{l}{Other Vendors} & -0.067 & -0.062 & 0.010 & -0.030 & -1.089*** & -0.139** \\
      &       & (0.048) & (0.111) & (0.129) & (0.033) & (0.325) & (0.077) \\
\multicolumn{1}{l}{6} & \multicolumn{1}{l}{Malt Beverage} & -0.037 & 0.008 & -0.037 & -0.036 & -0.057** & -2.126*** \\
      &       & (0.037) & (0.075) & (0.105) & (0.027) & (0.029) & (0.644) \bigstrut[b]\\
\hline
\multicolumn{8}{p{1.12\textwidth}}{Notes:
This table presents the estimated price elasticities by the main model, the time-invariant factor-augmented (TI-FA) bundle demand model with endogenous regressors (Endo).
Cell entries $(j,k)$, where $j$ indexes row and $k$ indexes column, give the posterior mean (and standard deviation in parentheses) of the percentage change in the probability of using $k$ substance in response to a percentage increase in the price of substance $j$.
*** $p<0.01$, ** $p<0.05$, * $p<0.1$.
The significance levels are based on the posterior credibility intervals.
} \bigstrut[t]\\
\end{tabular}

==> tables/elasticities_TV_FA_Endo.tex <==
\begin{tabular}{llcccccc}
\hline
\multicolumn{2}{r}{Good $k=$} & 1     & 2     & 3     & 4     & 5     & 6 \bigstrut[t]\\
Price $j=$ &       & AB InBev & Boston Beer & Heineken & MillerCoors & Other Vendors & Malt Beverage \bigstrut[b]\\
\hline
1     & AB InBev & -1.278*** & -0.058 & -0.025 & -0.036 & -0.024 & -0.018 \bigstrut[t]\\
      &       & (0.442) & (0.075) & (0.089) & (0.027) & (0.024) & (0.047) \\
2     & Boston Beer & -0.023 & -2.441*** & -0.044 & 0.001 & -0.020 & 0.003 \\
      &       & (0.026) & (0.844) & (0.083) & (0.016) & (0.018) & (0.032) \\
3     & Heineken & -0.006 & -0.027 & -2.257*** & -0.007 & -0.002 & -0.013 \\
      &       & (0.019) & (0.051) & (0.810) & (0.012) & (0.012) & (0.026) \\
4     & MillerCoors & -0.050 & 0.003 & -0.040 & -1.037*** & -0.022 & -0.064 \\
      &       & (0.040) & (0.070) & (0.084) & (0.359) & (0.026) & (0.057) \\
5     & Other Vendors & -0.053 & -0.115 & -0.016 & -0.035 & -1.426*** & -0.144** \\
      &       & (0.050) & (0.114) & (0.122) & (0.037) & (0.485) & (0.084) \\
6     & Malt Beverage & -0.016 & 0.006 & -0.045 & -0.042 & -0.059** & -2.321*** \\
      &       & (0.035) & (0.070) & (0.090) & (0.032) & (0.031) & (0.773) \bigstrut[b]\\
\hline
\multicolumn{8}{p{1.12\textwidth}}{Notes:
This table presents the estimated price elasticities by the main model, the time-varying factor-augmented (TV-FA) bundle demand model with endogenous regressors (Endo).
Cell entries $(j,k)$, where $j$ indexes row and $k$ indexes column, give the posterior mean (and standard deviation in parentheses) of the percentage change in the probability of using $k$ substance in response to a percentage increase in the price of substance $j$.
*** $p<0.01$, ** $p<0.05$, * $p<0.1$.
The significance levels are based on the posterior credibility intervals.
} \bigstrut[t]\\
\end{tabular}

==> tables/elasticities_TV_FA_Exo.tex <==
\begin{tabular}{llcccccc}
\hline
\multicolumn{2}{r}{Good $k=$} & 1     & 2     & 3     & 4     & 5     & 6 \bigstrut[t]\\
\multicolumn{1}{l}{Price $j=$} &       & AB InBev & Boston Beer & Heineken & MillerCoors & Other Vendors & Malt Beverage \bigstrut[b]\\
\hline
\multicolumn{1}{l}{1} & \multicolumn{1}{l}{AB InBev} & -1.117*** & -0.065 & 0.014 & -0.032 & -0.027 & -0.030 \bigstrut[t]\\
      &       & (0.394) & (0.076) & (0.098) & (0.025) & (0.023) & (0.046) \\
\multicolumn{1}{l}{2} & \multicolumn{1}{l}{Boston Beer} & -0.026 & -2.232*** & 0.002 & -0.001 & -0.013 & -0.003 \\
      &       & (0.026) & (0.802) & (0.091) & (0.016) & (0.018) & (0.032) \\
\multicolumn{1}{l}{3} & \multicolumn{1}{l}{Heineken} & 0.003 & 0.001 & -2.289*** & -0.006 & -0.001 & -0.009 \\
      &       & (0.020) & (0.056) & (0.850) & (0.013) & (0.013) & (0.028) \\
\multicolumn{1}{l}{4} & \multicolumn{1}{l}{MillerCoors} & -0.045 & -0.002 & -0.033 & -0.852*** & -0.017 & -0.057 \\
      &       & (0.036) & (0.068) & (0.088) & (0.300) & (0.023) & (0.051) \\
\multicolumn{1}{l}{5} & \multicolumn{1}{l}{Other Vendors} & -0.061 & -0.074 & -0.009 & -0.028 & -1.167*** & -0.111* \\
      &       & (0.049) & (0.110) & (0.125) & (0.034) & (0.407) & (0.074) \\
\multicolumn{1}{l}{6} & \multicolumn{1}{l}{Malt Beverage} & -0.027 & -0.007 & -0.031 & -0.037 & -0.046* & -2.091*** \\
      &       & (0.035) & (0.069) & (0.100) & (0.027) & (0.027) & (0.740) \bigstrut[b]\\
\hline
\multicolumn{8}{p{1.12\textwidth}}{Notes:
This table presents the estimated price elasticities by the main model, the time-varying factor-augmented (TV-FA) bundle demand model without endogenous regressors (Exo).
Cell entries $(j,k)$, where $j$ indexes row and $k$ indexes column, give the posterior mean (and standard deviation in parentheses) of the percentage change in the probability of using $k$ substance in response to a percentage increase in the price of substance $j$.
*** $p<0.01$, ** $p<0.05$, * $p<0.1$.
The significance levels are based on the posterior credibility intervals.
} \bigstrut[t]\\
\end{tabular}

==> tables/product_definition.tex <==
\begin{tabular}{llllc}
\hline
$j$   & Product & Vendor (Level 4) & Brand (Level 5) & Choice Probability \bigstrut\\
\hline
1     & Beer  & Anheuser-Busch InBev & Budweiser, Corona,… & 0.094 \bigstrut[t]\\
2     & Beer  & Boston Beer Company & Samuel Adams,… & 0.025 \\
3     & Beer  & Heineken USA & Heineken,… & 0.015 \\
4     & Beer  & MillerCoors & Coors, Miller Lite,… & 0.144 \\
5     & Beer  & Other Vendors & Sierra Nevada Pale Ale, Stone IPA,… & 0.177 \\
6     & Malt Beverage & All Vendors & Bacardi Silver Signature, Mike's Hard,… & 0.054 \bigstrut[b]\\
\hline
\multicolumn{5}{p{1.05\textwidth}}{Notes:
This table outlines the product definitions and monthly choice probabilities for beer and malt beverage products.
Products are divided into beer (including various types like ale, lager, pilsner, porter, stout) and malt beverage (including fruit-flavored beer and beer cocktails).
The choice probabilities indicate the average percentage of households purchasing a particular brand or product type within a month, based on household-level and store-level data from two BehaviorScan markets during the year 2011.
} \bigstrut[t]\\
\end{tabular}

==> tables/results_TV_FA_Endo.tex <==
\begin{tabular}{llcccccc}
\hline
      & \multicolumn{1}{r}{$j = $} & 1     & 2     & 3     & 4     & 5     & 6 \bigstrut[t]\\
      &       & AB InBev & Boston Beer & Heineken & MillerCoors & Other Vendors & Malt Beverage \bigstrut[b]\\
\hline
\multicolumn{8}{l}{\boldmath{}\textbf{Good Utility $\bar{u}_{ijt}$}\unboldmath{}} \bigstrut[t]\\
      & Price & \multicolumn{6}{c}{-0.373***} \\
      &       & \multicolumn{6}{c}{(0.126)} \\
      & Constant & -3.000*** & -6.194*** & -8.756*** & -1.571* & -1.991*** & -2.483** \\
      &       & (0.925) & (1.301) & (1.430) & (0.876) & (0.745) & (1.091) \\
      & No. of Shopping Trips & 0.058*** & 0.039*** & 0.036*** & 0.060*** & 0.058*** & 0.029*** \\
      &       & (0.007) & (0.008) & (0.011) & (0.006) & (0.005) & (0.007) \\
      & Household Income & 0.094 & 0.260*** & 0.407*** & 0.015 & 0.143*** & 0.077 \\
      &       & (0.074) & (0.098) & (0.085) & (0.065) & (0.047) & (0.069) \\
      & Cabled TV & -0.197 & 0.240 & 0.369 & 0.315*** & 0.110 & 0.092 \\
      &       & (0.133) & (0.213) & (0.219) & (0.132) & (0.101) & (0.140) \\
      & Pittsfield & 0.652*** & 1.517*** & 1.013*** & -0.816*** & -0.280 & 0.578*** \\
      &       & (0.164) & (0.152) & (0.181) & (0.154) & (0.201) & (0.157) \bigstrut[b]\\
\hline
\multicolumn{8}{l}{\boldmath{}\textbf{Bundle-Effects $\Gamma_{i(j_1,j_2)t}$}\unboldmath{}} \bigstrut[t]\\
      & Family Size (Demeaned) & \multicolumn{6}{c}{0.034***} \\
      &       & \multicolumn{6}{c}{(0.014)} \\
      & Boston Beer & 0.561*** &       &       &       &       &  \\
      &       & (0.153) &       &       &       &       &  \\
      & Heineken USA & 0.294*** & 0.518*** &       &       &       &  \\
      &       & (0.127) & (0.135) &       &       &       &  \\
      & MillerCoors & 0.566*** & 0.163 & 0.509*** &       &       &  \\
      &       & (0.083) & (0.146) & (0.154) &       &       &  \\
      & Other Vendors & 0.414*** & 0.516*** & 0.205 & 0.342*** &       &  \\
      &       & (0.072) & (0.105) & (0.125) & (0.062) &       &  \\
      & Malt Beverage & 0.295** & 0.156 & 0.479*** & 0.616*** & 0.774*** &  \\
      &       & (0.115) & (0.211) & (0.191) & (0.130) & (0.078) &  \bigstrut[b]\\
\hline
\multicolumn{8}{p{1.15\textwidth}}{Notes:
This table presents the posterior means and standard deviations (in parentheses) of the model parameters from the main specification, introduced in Subsection \ref{sec:data_and_specification}, and by the main model, the time-varying factor-augmented (TV-FA) bundle demand model with endogenous regressors.
*** $p<0.01$, ** $p<0.05$, * $p<0.1$. The significance levels are based on the posterior credibility intervals.
The upper panel details the good utility equations $\bar{u}_{ijt}$ for the six goods.
The six columns correspond to the six goods.
Note that the price coefficient $\alpha$ is common across all six utility equations.
The bottom panel details the bundle effects $\Gamma_{i(j_1,j_2)t}$ for all fifteen pairs of goods.
The coefficient on (demeaned) family size is assumed to be homogeneous across all pairs of bundles.
} \bigstrut[t]\\
\end{tabular}
